Interpreting and improving deep-learning models with reality checks

Recent deep-learning models have achieved impressive predictive performance by learning complex functions of many variables, often at the cost of interpretability. This chapter covers recent work aiming to interpret models by attributing importance to features and feature groups for a single prediction. Importantly, the proposed attributions assign importance to interactions between features, in addition to features in isolation. These attributions are shown to yield insights across real-world domains, including bio-imaging, cosmology image and natural-language processing. We then show how these attributions can be used to directly improve the generalization of a neural network or to distill it into a simple model. Throughout the chapter, we emphasize the use of reality checks to scrutinize the proposed interpretation techniques.

==> figs_cdep/sst_example3.tex <==
{\large \textbf{Positive}}
{\small
	
% {\fontfamily{qcs}\selectfont 
pacino is the best \pos{she}'s been in years and keener is marvelous 

\pos{she} showcases davies as a young woman of great charm, generosity and diplomacy

% shows \pos{she}'s back in form, with an astoundingly rich film.

% proves once again that \pos{she}'s the best brush in the business

}
\vspace{0.2cm}
% }
{\large \textbf{Negative}}

% {\fontfamily{qcs}\selectfont 
{\small
% green ruins every single scene \nega{he}'s in, and the film, while it's not completely wreaked, is seriously compromised by that

i'm sorry to say that this should seal the deal - arnold is not, nor will \nega{he} be, back.

this is sandler running on empty, repeating what \nega{he}'s already done way too often.

% so howard appears to have had free rein to be as pretentious as \nega{he} wanted
}

% }
	
